The Adaptive Multi-Factor Model and the Financial Market

Modern evolvements of the technologies have been leading to a profound influence on the financial market. The introduction of constituents like Exchange-Traded Funds, and the wide-use of advanced technologies such as algorithmic trading, results in a boom of the data which provides more opportunities to reveal deeper insights. However, traditional statistical methods always suffer from the high-dimensional, high-correlation, and time-varying instinct of the financial data. In this dissertation, we focus on developing techniques to stress these difficulties. With the proposed methodologies, we can have more interpretable models, clearer explanations, and better predictions.

==> commondefs <==
#
# Rules and definitions for building various things, especially 
# TeX documents.
# -- Andrew Myers
# Last updated April 2007
#

MAKEDIR = .
INCLDIR = .
TEXDIR = .

COMMONRULES = $(MAKEDIR)/commonrules

SOURCES = $(CFILES) $(C++FILES) $(YFILES) $(LFILES) $(AFILES)
OBJECTS = $(CFILES:.c=.o) $(C++FILES:.C=.o)
DIRT = *.o core *.aux *.dvi *.log *.stamp *.i *.bbl *.[ib]lg $(LDIRT)
GENERATED = .dependtime Makedepend Makedepend.bak
RM = rm -f
MKDEPFILE = Makedepend
MKDEPEND = makedepend
MKDEPFLAGS = -Y
MKDEPC++FLAGS = $(C++DEFS) $(C++INCS) $(MKDEPFLAGS)
MKDEPCFLAGS = $(CDEFS) $(CINCS) $(MKDEPFLAGS)

.SUFFIXES: .C .ps .i .txt .h
.SUFFIXES: .tex .dvi .ind .idx .bbl .aux .glo .aux .stamp .pdf .eps

GNUBIN = /usr/local

ATTC++ = CC
DECC++ = cxx
GNUC++ = g++

CC = cc
C++ = $(GNUC++)
YACC = bison
DVIPS = dvips

C++F = $(C++) $(C++FLAGS)
CCF = $(CC) $(CFLAGS)

C++FLAGS = $(C++OPTS) $(C++DEFS) $(C++INCS)

C++INCS = $(GC++INCS) $(LC++INCS)
C++OPTS = $(GC++OPTS) $(LC++OPTS)
C++DEFS = $(GC++DEFS) $(LC++DEFS)

GC++OPTS = $(OPTIMIZER)

CFLAGS = $(COPTS) $(CDEFS) $(CINCS)
COPTS = $(GCOPTS) $(LCOPTS)
CDEFS = $(GCDEFS) $(LCDEFS)
CINCS = $(GCINCS) $(LCINCS)

GCOPTS = $(OPTIMIZER)

M3F = $(M3) $(M3FLAGS)
M3 = m3
M3PP = m3pp

LDFLAGS = $(LLDFLAGS) $(GLDFLAGS)
LLDFLAGS = $(LLDLIBS) $(LLDOPTS) 

SEP=:
#SEP=\;         # for MikTeX+Cygwin
TEXINPUTS = .$(SEP)$(TEXDIR)$(SEP)
LATEX = TEXINPUTS=$(TEXINPUTS) latex
PDFLATEX = TEXINPUTS=$(TEXINPUTS) pdflatex


==> commonrules <==
# Some basic recursive rules for building, installing, and cleaning up
# a source tree
#
subdirs:
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make); \
	fi; done;

clean:  localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

localclean:
	$(RM) $(DIRT)

clobber: localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;
	$(RM) $(TARGETS) $(GENERATED)

install: default localinstall
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

incdepend: .dependtime
depend: .dependtime

.dependtime: $(SOURCES)
	touch temp
	$(MKDEPEND) $(MKDEPC++FLAGS) -f temp $(C++FILES)
	touch $(MKDEPFILE)
	$(MKDEPEND) $(MKDEPCFLAGS) -f $(MKDEPFILE) $(CFILES)
	cat temp >> $(MKDEPFILE)
	rm -f temp
	touch $@

# Rules for TeX files
#
# The line that runs LATEX needs to run inside a subshell to turn off
# "make"'s status checking. It blows away .aux because the .aux file
# created is bad and also breaks bibtex. It touches .stamp to force a
# rebuild.
.tex.dvi:
	@if test -r "$*.aux"; \
	   then cp $*.aux $*.auxprev; \
	   else echo > $*.auxprev; \
	fi
	@echo "$(LATEX) $<"
	@sh -c "$(LATEX) $< || (rm -f $*.aux; sleep 1; touch $*.stamp; exit 1)"
	@-cmp -s $*.aux $*.auxprev; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch $*.stamp; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f $*.auxprev

.tex.pdf:
	@if test -r "$*.aux"; \
	   then cp $*.aux $*.auxprev; \
	   else echo > $*.auxprev; \
	fi
	@echo "$(PDFLATEX) $<"
	@sh -c "$(PDFLATEX) $< || (rm -f $*.aux; sleep 1; touch $*.stamp; exit 1)"
	@-cmp -s $*.aux $*.auxprev; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch $*.stamp; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f $*.auxprev

# must add dependencies like
#    foo.ind: foo.stamp
#    foo.dvi: foo.ind
# to use this rule properly.
.tex.ind:
	@if [ -f $*.idx ]; then \
	   echo makeindex $*.idx; \
	   makeindex $*.idx; \
	else \
	   echo touch $@; \
	   touch $@; \
        fi

# must add dependencies like
#    foo.bbl: foo.bib
#    foo.dvi: foo.bbl
# to use this rule properly.
.tex.bbl:
	@if [ -r $*.aux ]; then echo bibtex $*; sh -c "bibtex $(BIBOPTS) $* || echo"; else echo; fi

.tex.stamp: # backward compatibility
	touch $@

.dvi.ps:
	$(DVIPS) $(DVIPSOPTS) $< -o $@
.eps.pdf:
	epstopdf $<

#
# Rules for C++ and .i files
#

.C.i:
	$(C++F) -E $< > $@

.c.i:
	$(CCF) -E $< > $@

.C.o:
	$(C++F) -c $<

# include $(M3SU)    # old Modula-3 rules

